Third-Party Hardware IP Assurance against Trojans through Supervised Learning and Post-processing

System-on-chip (SoC) developers increasingly rely on pre-verified hardware intellectual property (IP) blocks acquired from untrusted third-party vendors. These IPs might contain hidden malicious functionalities or hardware Trojans to compromise the security of the fabricated SoCs. Recently, supervised machine learning (ML) techniques have shown promising capability in identifying nets of potential Trojans in third party IPs (3PIPs). However, they bring several major challenges. First, they do not guide us to an optimal choice of features that reliably covers diverse classes of Trojans. Second, they require multiple Trojan-free/trusted designs to insert known Trojans and generate a trained model. Even if a set of trusted designs are available for training, the suspect IP could be inherently very different from the set of trusted designs, which may negatively impact the verification outcome. Third, these techniques only identify a set of suspect Trojan nets that require manual intervention to understand the potential threat. In this paper, we present VIPR, a systematic machine learning (ML) based trust verification solution for 3PIPs that eliminates the need for trusted designs for training. We present a comprehensive framework, associated algorithms, and a tool flow for obtaining an optimal set of features, training a targeted machine learning model, detecting suspect nets, and identifying Trojan circuitry from the suspect nets. We evaluate the framework on several Trust-Hub Trojan benchmarks and provide a comparative analysis of detection performance across different trained models, selection of features, and post-processing techniques. The proposed post-processing algorithms reduce false positives by up to 92.85%.

==> feature.tex <==

\textbf{Static Probability Extraction Technique:}
We observed that simulation based probability calculation gets significantly affected by the types of test vectors as well as the number of total vectors. Hence , we have used vector-less approach to derive the signal probability of each net in the design. 
% Though, the simulation based calculations which are done for a reasonably long duration with realistic stimulus are good, 
The vector-less probability feature calculations are an excellent compromise between accuracy and compute efficiency compared to the simulation based calculations that are done for a reasonably long duration with realistic stimulus. To derive the signal probability of a net in a gate-level designs, the hyper-graph representation of the gate level Verilog design is obtain by parsing the Verilog netlist. For all the features that are used to train an ML model, the features are extracted by considering sequential elements as full-scan flip-flops. With this assumption, the outputs of the sequential elements are considered as pseudo-primary input and inputs of the sequential elements are considered as pseudo-primary outputs. This assumption enables us to perform topological sort on the hyper-graph provided there are no combinational loops in the original design. Finally, the hyper-graph is traversed using topologically sorted nodes from inputs to outputs while evaluating the signal probability features of each net using table \ref{tab:stat_prob}. 
% \textcolor{red}{Table reference not matching.} 
The static probability of all the nets is within the range 0 to 1. If the static probability of a net being at logic-1 is 1, it suggests that the net is held at Logic 1 for entire operation and if it is 0, it suggests that the chances of net being held at logic 1 is very low or 0. If a design has an active high reset with Static probability of being 1 is 0.9 implies that the reset is active 90\% of the time. 
% reference vivado user manual
Rarely switching Trojan nets should have nets with very low or very high signal probability of either 0 or 1.

\begin{table}[h]
\centering
\label{tab:stat_prob}
\caption{Static Probability of basic gates}
\begin{tabular}{|c|l|l|}  \hline
 \textbf{\#} & \multicolumn{1}{|c|}{\textbf{Gate}} & \multicolumn{1}{|c|}{\textbf{Signal Probability of 1}}                \\ \hline
1          & NOT    & {$1 - P_A$}        \\  \hline
2          & AND    & {$P_A*P_B$}        \\  \hline
3          & OR     & {$P_A + P_B - P_A*P_B$}        \\  \hline
\end{tabular}
\end{table}

\\ \textbf{Transition Probability:} %The toggle rate (also referred to as transition rate) is the number of transitions per unit time (i.e., seconds).  For instance, if the signal toggles 4 times in 40 ns, it translates to: $\dfrac{4}{40*10^{-9}}$= 100 million transitions per second (Mtr/s). 
The transition probability (also referred to as toggle rate or activity) is the number of transitions from logical level 0 to 1 or 1 to 0. 

\textbf{Extraction Technique:}
Transition probability can be obtained by either simulating set of test vectors or with a vector-less approach. In simulation approach, the transition probability gets affected by the order in which vectors are passed while performing the simulation. For instance, if two consecutive vectors used during simulation differs by only one bit, then the chances of observing transition on the nets that are affected by this bit change are low. Hence, for transition probability feature as well we have used vector-less approach to derive transition probability for each net in the design which considers type of gate driving a particular net to derive the feature value. For transition probability feature, hyper-graph is traversed in the topological order while evaluating feature for each net. Here, as we have opened the design with full-scan assumption, the approach does not have to deal with the feedback signals. For compute efficiency, re-convergent fan-outs are not considered while evaluating the feature values. If, the transition probability of transitioning a signal from 0 to 1 is high it implies that the signal toggles multiple time between logic level 0 and 1. In sequential design, the transition probability of clock signal to transition from 0 to 1 or 1 to 0 will be a high number. Hard-to-activate Trojans are likely to contain nets with very low transition probability. To evaluate the transition probability of each gate in a design, table \ref{tab:trans_prob2} is referred.


% \begin{table}[h]
% \centering
% \label{tab:trans_prob1}
% \caption{\textcolor{red}{choose 1}Transition Probability of basic gates}

% \begin{tabular}{|c|l|l|}  \hline
%  \textbf{\#} & 
%  {\textbf{Gate}} & 
%  {\textbf{ \begin{math} P_{0 to 1} = P_{out=0} * P_{out=1} \end{math}}}     \\ \hline
% 1   & NOT    & {\(1-P_A\)*\(P_A\)}                                           \\  \hline
% 2   & AND    & {\(1-P_A*P_B\)*\(P_A*P_B\)}                                   \\  \hline
% 3   & OR     & {\begin{math}(1-P_A)*(1-P_B)*(1-(1-P_A)*(1-P_B))\end{math}}                   \\  \hline
% 4   & NAND   & {\begin{math}(P_A*P_B)*(1-P_A*P_B)\end{math}}                                 \\  \hline
% 5   & NOR    & {\begin{math}(1-(1-P_A)*(1-P_B))*(1-P_A)*(1-P_B)\end{math}}                   \\  \hline
% 6   & XOR    & {\begin{math}(1-(P_A + P_B - 2*P_A*P_B))*\end{math} \\ 
%     &        &  \begin{math}(P_A + P_B - 2*P_A*P_B)\end{math}} \\  \hline
% \end{tabular}
% \end{table}

\begin{table}[h]
\centering
\label{tab:trans_prob2}
% \caption{\textcolor{red}{choose 1}Transition Probability of basic gates}
\caption{Transition Probability of basic gates}

\begin{tabular}{|c|l|l|}  \hline
 \textbf{\#} & 
 {\textbf{Gate}} & 
 {\textbf{ \begin{math} P_{0 to 1} = P_{out=0} * P_{out=1} \end{math}}}     \\ \hline
1   & NOT    & {\(1-A\)*\(A\)}                                           \\  \hline
2   & AND    & {\(1-A*B\)*\(A*B\)}                                   \\  \hline
3   & OR     & {\begin{math}(1-A)*(1-B)*(1-(1-A)*(1-B))\end{math}}                   \\  \hline
4   & NAND   & {\begin{math}(A*B)*(1-A*B)\end{math}}                                 \\  \hline
5   & NOR    & {\begin{math}(1-(1-A)*(1-B))*(1-A)*(1-B)\end{math}}                   \\  \hline
6   & XOR    & {\begin{math}(1-(A + B - 2*A*B))*(A + B - 2*A*B)\end{math}} \\  \hline
\end{tabular}
\end{table}

% \textcolor{red}{
% \\ \textbf{Entropy:} Each net except the primary inputs in a gate-level design is driven by a cell (gate or flip-flop). %The cell could be a flip-flop (FF) or a combinational logic. 
% Entropy is a measure of balance in the number of zeros and ones in its truth table of the cell. 
% If the probability of 1 and 0 in the output column of a truth table is $P_{1}$ and $P_{0}$ respectively, the entropy of the cell is calculated as: 
% $$E=P_{1} \log_2 \dfrac{1} {P_{1}}  + P_{0} \log_2 \dfrac{1} {P_{0}}$$ 
% %For FFs, the entropy value is defined similarly to a single input buffer logic mapped onto a LUT. 
% The entropy of the cell provides various aspects regarding its functional behaviour. For instance, if the output column of the truth table mostly contains zeros, the functionality of the corresponding gate resembles to an AND function. Even though an attacker can construct the same malicious functionality with different types of gate structures to bypass identification, the underlying behaviour of the logic should be the same when observed using such functional features. In \cite{hoque2018hardware}, the authors used entropy in FPGA-mapped designs where nets are driven by LUTs that usually contain large combinational logic functions. However, in gate-level designs a large portion of nets are driven by cells with small number of inputs. Hence, disjointed observation of entropy of each cell may provide limited information in learning and identifying a malicious circuit containing a group of cell. Therefore, we augment entropy as a neighborhood feature that provides the entropy information of the surrounding nets as well.}


% \begin{algorithm}
% 	\caption{Feature extraction with full-scan assumption}
%         \label{alg:full_scan_algo}
%     \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
% 	\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
% 	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% 		\Input{ $d$: Gate-level netlist. \\ } 
% 		\Output{$vipr\_features$: Features for each individual net in the design.}
% 		\ForEach { $net$ in $d$}
% 		{
% 		    \If{ ($net$ is in $Primary Inputs$ or $net$ is in $Pseudo-Primary Inputs$) }
% 		    {
% 		        SP1(net) = 0.5  \\
%         		SP0(net) = 0.5  \\
%         		CC0(net) = 1    \\
%         		CC1(net) = 1    \\
% 		    }
% 		    \If{ ($net$ is in $Primary Outputs$ or $net$ is in $Pseudo-Primary Outputs$) }
% 		    {
% 		        CO(net) = 0     \\
%         		SO(net) = 0     \\
% 		    }
% 		}
% 		\ForEach { $node$ in $topoSortNodes$}{
% 	        Evaluate\_SP(node)   \\
% 	        Evaluate\_TP(node)   \\
% 	        Evaluate\_CC(node)   \\
% 	    }
% 	    \ForEach { $node$ in reversed($topoSortNodes$)}{
% 	        Evaluate\_CO(node)   \\
% 	    }
%      \textbf{return} $connectedList$
% \end{algorithm}\DecMargin{1em}


\textbf{Controlability and Observability Extraction Technique:}
We have implemented two variations of SCOAP measure. Because of full-scan assumption of sequential elements, we have obtained combinational SCOAP values for each of the net in the gate-level design. In second approach, we have extracted SCOAP measure with no-scan assumption as per \cite{scoap_sandia}. 

To evaluate combinational SCOAP with full-scan assumption, the hyper-graph is topologically sorted with the help of full-scan assumption. The combinational SCOAP features which are calculated with the help of \ref{tab:comb_cc}, \ref{tab:comb_obs}. Here, combinational 0-controllability and 1-controllability of inputs are set to (1, 1) and combinational observability of outputs is set to 0. Then the hyper-graph is traversed from input to outputs while evaluating the combinational controllability feature values based on type of the cell. To extract the combinational observability, the hyper-graph is traversed from output to inputs and combinational observability features are evaluated based on type of the cell, observability of the output of the cell and combinational controllability of the inputs of the current cell.  

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/scoap_gate_3.png}
    \caption{Example 'AND' gate with its combinational controllability to 0/1 and combinational observability feature value}
    \label{fig:scoap_gate}
\end{figure}

To evaluate SCOAP measure with all flip-flop as non-scan flip-flops algorithm mentioned \cite{scoap_sandia} is used. For figure \ref{fig:and_gate}, the combinational 0-controllability of the output depends on how difficult it is to make the output of the 'AND' gate to logic-0. This can be done by either controlling input a to logic-0 or input b to logic-0. Hence, the first equation for 'AND' gate shown in table \ref{tab:comb_cc} considers minimum value of controlling either of inputs to logic-0 and 1 is added to consider the logic level of the cell in the design. Similarly, to set the output z at logic-1, we need to control both of the inputs to logic-1. This combinational 1-controllability of the 'AND' gate is calculated as shown in \ref{tab:comb_cc} . In general, we need to control inputs of the driving cell to calculate the controllability of any output net to either 1 or 0. To evaluate combinational observability of input a of the 'AND' gate, we should be able to first observe value at the output of the cell and at the same time we should be able to control the input b of the cell to its non-controlling value as shown in \ref{tab:comb_obs} In case of fanout stem, the minimum observability of all the stems is considered as the final observability value as the fanout stem can be observed if any of the fanout nets are observed and to observe the effect quickly minimum value is considered. 

\begin{table}[h]
\centering
\label{tab:comb_cc}
\caption{Combinational Controllability of basic gates}
\begin{tabular}{|c|l|l|}  \hline
\textbf{\#} & \multicolumn{1}{|c|}{\textbf{Gate}}   & \multicolumn{1}{|c|}{\textbf{ Controllability }}    \\ \hline
\multirow{2}{*}{1}      &   \multirow{2}{*}{NOT}  & {CC0(z) = CC1(a) + 1}                                 \\
                        &                         & {CC1(z) = CC0(a) + 1}                                 \\  \hline
\multirow{2}{*}{2}      &   \multirow{2}{*}{AND}  & {CC0(z) = min(CC0(a), CC0(b)) + 1}                    \\
                        &                         & {CC1(z) = CC1(a) + CC1(b) + 1}                        \\  \hline
\multirow{2}{*}{3}      &   \multirow{2}{*}{OR}   & {CC0(z) = CC0(a) + CC0(b) + 1}                        \\
                        &                         & {CC1(z) = min(CC1(a), CC1(b)) + 1}                    \\  \hline
\multirow{2}{*}{4}      &   \multirow{2}{*}{NAND} & {CC0(z) = CC1(a) + CC1(b) + 1}                        \\
                        &                         & {CC1(z) = min(CC0(a), CC0(b)) + 1}                    \\  \hline
\multirow{2}{*}{5}      &   \multirow{2}{*}{NOR}  & {CC0(z) = min(CC1(a), CC1(b)) + 1}                    \\
                        &                         & {CC1(z) = CC0(a) + CC0(b) + 1}                        \\  \hline
\multirow{2}{*}{6}      &   \multirow{2}{*}{XOR}  & {CC0(z) = min(CC0(a) + CC0(b), CC1(a) + CC1(b)) + 1}  \\
                        &                         & {CC1(z) = min(CC1(a) + CC0(b), CC0(a) + CC1(b)) + 1}  \\  \hline
\multirow{2}{*}{7}      &   \multirow{2}{*}{XNOR} & {CC0(z) = min(CC1(a) + CC0(b), CC0(a) + CC1(b)) + 1}  \\
                        &                         & {CC1(z) = min(CC0(a) + CC0(b), CC1(a) + CC1(b)) + 1}  \\  \hline
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\label{tab:comb_obs}
\caption{Combinational Observability of basic gates}
\begin{tabular}{|c|l|l|}  \hline
\textbf{\#} & \multicolumn{1}{|c|}{\textbf{Gate}}   & \multicolumn{1}{|c|}{\textbf{ Observability }}    \\ \hline
\multirow{2}{*}{1}      &   \multirow{2}{*}{NOT}  & {CO(a) = CO(z) + 1}                                 \\
                        &                         & {CO(a) = CO(z) + 1}                                 \\  \hline
\multirow{2}{*}{2}      &   \multirow{2}{*}{AND}  & {CO(a) = CO(z) + CC1(b) + 1}                        \\
                        &                         & {CO(b) = CO(z) + CC1(a) + 1}                        \\  \hline
\multirow{2}{*}{3}      &   \multirow{2}{*}{OR}   & {CO(a) = CO(z) + CC0(b) + 1}                        \\
                        &                         & {CO(b) = CO(z) + CC0(a) + 1}                        \\  \hline 
\multirow{2}{*}{4}      &   \multirow{2}{*}{NAND} & {CO(a) = CO(z) + CC1(b) + 1}                        \\
                        &                         & {CO(b) = CO(z) + CC1(a) + 1}                        \\  \hline
\multirow{2}{*}{5}      &   \multirow{2}{*}{NOR}  & {CO(a) = CO(z) + CC0(b) + 1}                        \\
                        &                         & {CO(b) = CO(z) + CC0(a) + 1}                        \\  \hline
\multirow{2}{*}{6}      &   \multirow{2}{*}{XOR}  & {CO(a) = CO(z) + min(CC0(b), CC1(b)) + 1}           \\
                        &                         & {CO(b) = CO(z) + min(CC0(a), CC1(a)) + 1}           \\  \hline
\multirow{2}{*}{7}      &   \multirow{2}{*}{XNOR} & {CO(a) = CO(z) + min(CC0(b), CC1(b)) + 1}           \\
                        &                         & {CO(b) = CO(z) + min(CC0(a), CC1(a)) + 1}           \\  \hline
8           & STEM      & {CO(a) = min(CO(z1), CO(z2), ..., CO(zn))}                                    \\  \hline
\end{tabular}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/scoap_fig_5.png}
    \caption{Initialization  for computing  Sandia SCOAP feature extraction}
    \label{fig:sandia_scoap}
\end{figure}

To evaluate SCOAP measure with non-scan assumption, SCOAP equations for different types of flip-flops are derived based on the functionality of the flip-flop. For example, in figure \ref{fig:sandia_scoap}, assume that the flip-flop is a negative edge triggered flip-flop. As shown in equation 1-2 for combinational and sequential 1-controllability, we need to control the 'q' output of the flip-flop to logic value of 1. To acheive this we need to control 'd' input of the flip-flop to 1 and make a negative transition on the 'clk' input. 

\begin{equation}
    \label{CC1_Q_equation}
    CC_1(q) = CC_1(d) + CC_1(clk) + CC_0(clk)
\end{equation}

\begin{equation}
    \label{SC_1_equation}
    SC_1(q) = SC_1(d) + SC_1(clk) + SC_0(clk) + 1
\end{equation}


% $CC1(Q) = CC1(DIN) + CC1(CLK) + CC0(CLK)$  \\
% $SC1(Q) = SC1(DIN) + SC1(CLK) + SC0(CLK) + 1$  \\

Similarly, to control the 'q' output of the flip-flop to logic value of 0, control 'd' input of the flop to 0 and make a negative transition on the 'clk' input as shown in equation 3-4. 

\begin{equation}
    \label{CC0_Q_equation}
    CC_0(q) = CC_0(d) + CC_1(clk) + CC_0(clk) 
\end{equation}

\begin{equation}
    \label{CC1_Q_equation}
    SC_0(q) = SC_0(d) + SC_1(clk) + SC_0(clk) + 1
\end{equation}

% $CC0(Q) = CC0(DIN) + CC1(CLK) + CC0(CLK)$  \\
% $SC0(Q) = SC0(DIN) + SC1(CLK) + SC0(CLK) + 1$  \\

Now, to observe the 'd' line, we should be able to observe 'q' output of the flip-flop and additionally we need to set the 'q' output to 0, generate a falling edge on the 'clk' signal The resulting equation for the observability of the 'd' input of the flip-flop is shown in equations 5-6.

\begin{equation}
    \label{CC1_Q_equation}
    CO(d) = CO(q) + CC_0(q) + CC_1(clk) + CC_0(clk)
\end{equation}

\begin{equation}
    \label{CC1_Q_equation}
    SO(d) = SO(q) + SC_0(q) + SC_1(clk) + SC_0(clk) + 1
\end{equation}

% $CO(DIN) = CO(Q) + CC0(Q) + CC1(CLK) + CC0(CLK)$ \\
% $SO(DIN) = SO(Q) + SC0(Q) + SC1(CLK) + SC0(CLK) + 1$ \\

Next, to observe the 'clk' line, we need either need to set the 'q' output to logic 1 and clock in logic 0 from 'd' input or set the 'q' output to logic 0 and clock in logic 1 from 'd' input as shown in equations 7-8.

\begin{multline}
    CO(clk) = CO(q) + CC_1(clk) + CC_0(clk) + \\
            min\{CC_1(q) + CC_0(d), CC_0(q) + CC_1(d)\} \\
\end{multline}

\begin{multline}
% \begin{equation}
    SO(clk) = SO(q) + SC_1(clk) + SC_0(clk) + \\
    min\{SC_1(q) + SC_0(d) , SC_0(q) + SC_1(d)\} + 1   \\
% \end{equation}
\end{multline}

% \begin{equation*}
%     \label{CC1_Q_equation}
%     SO(clk) = min\{SO(q) + SC_1(q) + SC_0(d) + SC_1(clk) + SC_0(clk), SO(q) + SC_0(q) + SC_1(d) + SC_1(clk) + SC_0(clk) + 1   \\
% \end{equation*}

% $CO(CLK) = min\{CO(Q) + CC1(Q) + CC0(DIN) + CC1(CLK) + CC0(CLK), CO(Q) + CC0(Q) + CC1(DIN) + CC1(CLK) + CC0(CLK)\}$ \\ 
% $SO(CLK) = min\{SO(Q) + SC1(Q) + SC0(DIN) + SC1(CLK) + SC0(CLK), SO(Q) + SC0(Q) + SC1(DIN) + SC1(CLK) + SC0(CLK) + 1\}$    \\

While evaluating SCOAP features with no-scan assumption, each combinational controllablity feature value is incremented by 1 if feature is being evaluated for a combinational cell. Similarly, for sequnetial controllability measure, feature value is incremented by 1 if the feature is being evaluated for a sequential cell.

Combinational and sequential controllability of 0 or 1 is combined as shown in equations 9-10.\\

\begin{equation}
    \label{CC_equation}
    CC = \sqrt{CC_0^2 + CC_1^2}    \\  
\end{equation}

\begin{equation}
    \label{SC_equation}
    SC = \sqrt{SC_0^2 + SC_1^2}    \\
\end{equation}

Some of the previous works on hardware Trojan detection relies on Synopsys's TetraMax tool to extract the SCOAP measure. One of the limitations of the TetraMax tool is that the maximum value that the tool can assign to a net is limited to 254. So for nets that can have values greater than 254 gets assigned with asterisk symbol. Hence, we have not used the TetraMax tool to extract this feature as the SCOAP values can go beyond the set threshold present in TetraMax. Publicly available "Testability Measurement Tool" does not support designs in Verilog format and for designs which consists of loops, an infinity value is returned. In the recent work presented in 
% CITE SC-COTD paper, 
feature values for some of the flip-flops are passed as it is from input to output. This will impact the final feature values. Hence, we have implemented the algorithm to from scratch to evaluate the SCOAP features for non-scan assumption of the design. Here, we have assigned 10,000 as the maximum SCOAP value for all nets in the design which are not the primary input or outputs of the design. Then algorithm present in \cite{scoap_sandia} is used to calculate the feature values for all the nets.

To design a Trojan that is hard to activate during logic testing, an attacker is expected to design the trigger mechanism using nets with low controllability (i.e. higher controllability measure). To further hide the Trojan, the corresponding payload could be designed to impact only low observable (i.e. high observability measure) nodes. These two features have been used for detecting Trojans using unsupervised clustering \cite{salmani2016cotd}. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/and_gate.png}
%     % \caption{Example 'AND' gate with its combinational controllability to 0/1 and combinational observability feature value}
%     \label{fig:and_gate}
% \end{figure}



% \textbf{Control Value of Input:} 
% Control value represents the degree of control that an input to a Boolean function has on determining the state of its output. Observation of control values of inputs driving a net could be useful to identify the presence of nearly-unused or stealthy input signals at the fanin of that net.
% In \cite{hoque2018hardware}, the authors used the average, minimum, maximum, and standard deviation of control values of all inputs to the LUT driving the net as features. We calculate these four features for each cell in the gate-level design.

%While the observation of control values in a large function with many inputs may help to identify the presence of nearly-unused or stealthy input signals, when considering individual cells in a gate-level design the observation could become very localized. Hence, we integrated the control values of the connected signals.  



